RAG-Instruct: Boosting LLMs with Diverse Retrieval-Augmented Instructions

Retrieval-Augmented Generation (RAG) has emerged as a key paradigm for enhancing large language models (LLMs) by incorporating external knowledge. However, current RAG methods face two limitations: (1) they only cover limited RAG scenarios. (2) They suffer from limited task diversity due to the lack of a general RAG dataset. To address these limitations, we propose RAG-Instruct, a general method for synthesizing diverse and high-quality RAG instruction data based on any source corpus. Our approach leverages (1) five RAG paradigms, which encompass diverse query-document relationships, and (2) instruction simulation, which enhances instruction diversity and quality by utilizing the strengths of existing instruction datasets. Using this method, we construct a 40K instruction dataset from Wikipedia, comprehensively covering diverse RAG scenarios and tasks. Experiments demonstrate that RAG-Instruct effectively enhances LLMs' RAG capabilities, achieving strong zero-shot performance and significantly outperforming various RAG baselines across a diverse set of tasks. RAG-Instruct is publicly available at https://github.com/FreedomIntelligence/RAG-Instruct.

==> prompt/p1.tex <==

\begin{prompt}[title={Useless Doc}] \label{prompt_r0}
\{<provided text>\}

Please create an English question-answer pair based on the provided \texttt{<text>}. Please note that the question can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats.
You need to follow the following rules to generate the question:

1. The generated question is related to the \texttt{<text>}, but the \texttt{<text>} does not provide any helpful information to answer it.

2. Follow the question type of the example question below.

3. Please ensure that both the type and style for the generated questions are as diverse as possible. The richer the variety, the better.

Example: \texttt{\{example question\}}

Then, independently generate an answer to this question without being influenced by the \texttt{<text>}. Please make sure your answer is detailed, and try to include reasoning processes or evidence for your answer.

Please directly generate the question-answer pair following the rules above and in the format of \texttt{\{"Question": ..., "Answer": ...\}}.
\end{prompt}

\begin{prompt}[title={Single-Doc Support}] \label{prompt_r1}
\{<provided text>\}

Please generate an English question-answer pair according to the provided \texttt{<text>}. Please note that the question can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats.
You need to follow the following three rules to generate the question:

1. For the question, the \texttt{<text>} does not contain the answer, but is helpful for answering it.

2. Follow the question type of the example question  below.

3. Please ensure that both the type and style for the generated questions are as diverse as possible. The richer the variety, the better.

Example: \texttt{\{example question\}}

Then you need to generate an answer to the question based on the content of the provided \texttt{<text>}. Please make sure your answer is detailed, and try to include reasoning processes or evidence for your answer.

Please directly generate the question-answer pair following the rules above and in the format of \texttt{\{"Question": ..., "Answer": ...\}}.
\end{prompt}



\begin{prompt}[title={Multi-Doc Support}] \label{prompt_r2}
\{<provided texts>\}

Please generate an English question-answer pair according to the provided \texttt{<text>s}. Please note that the question can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats.
You need to follow the following rules to generate the question:

1. For the question, both \texttt{<text>s} do not contain the answer, but are helpful for answering it.

2. Follow the question type of the example question below.

3. Please ensure that both the type and style for the generated questions are as diverse as possible. The richer the variety, the better. 

4. Make sure that the final question is a single question, not a simple combination of multiple questions. 


Example: \texttt{\{example question}\}

Then, you need to generate an answer that utilizes or references the content of both \texttt{<text>s} to answer the generated question. Ensure the answer incorporates not only the information from the \texttt{<text>s} but also your own reasoning and knowledge. Please make sure your answer is detailed, and try to include reasoning processes or evidence for your answer.

Please directly generate the question-answer pair following the rules above and in the format of \texttt{\{"Question": ..., "Answer": ...\}}.
\end{prompt}



\begin{prompt}[title={Single-Doc Answer}]\label{prompt_r3}
\{<provided text>\}

Your task is to generate an English question-answer pair according to the provided \texttt{<text>}. Please note that the question can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats.
You need to follow the following three rules to generate the question:


1. Ensure that the answer to the generated question appears directly in the \texttt{<text>} or can be answered using the content from the \texttt{<text>}.

2. Follow the question type of the example question below.

3. Please ensure that both the type and style for the generated questions are as diverse as possible. The richer the variety, the better.

Example: \texttt{\{example question}\}

Then you need to generate an answer to the question based on the content of the provided \texttt{<text>}. Please make sure your answer is detailed, and try to include reasoning processes or evidence for your answer.

Please directly generate the question-answer pair following the rules above and in the format of \texttt{\{"Question": ..., "Answer": ...\}}.
\end{prompt}




\begin{prompt}[title={Multi-Doc Answer}]
\label{prompt_r4}
\{<provided texts>\}

Your task is to generate an English question-answer pair according to the provided \texttt{<text>s}. Please note that the question can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats.
You need to follow the following rules to generate the question:

1. Ensure that the answer to the generated question appears directly in both \texttt{<text>s} or can be answered using the content from both \texttt{<text>s}.

2. Follow the question type of the example question below.

3. Please ensure that both the type and style for the generated questions are as diverse as possible. The richer the variety, the better.

4. Make sure that the final question is a single question, not a simple combination of multiple questions. 


Example: \texttt{\{example question}\}

Then you need to generate an answer to the question based on the content of both \texttt{<text>s}. Please make sure your answer is detailed, and try to include reasoning processes or evidence for your answer.

Please directly generate the question-answer pair following the rules above and in the format of \texttt{\{"Question": ..., "Answer": ... \}}.
\end{prompt}


==> prompt/p2.tex <==
\begin{figure*}[ht!]
\centering

\begin{prompt}[title={Useless Doc ($r_0$)}] \label{prompt_r0}
<Documents> \newline
[1] \texttt{\{<Document 1>\}}\newline
</Documents> \newline

Your task is to generate an English question q* and a corresponding response a* based on the provided <Documents>. Please note that the question q* can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats. You need to follow the requirements below to generate the q* and a* \textcolor{blue}{(RAG Paradigms)}:  

\textcolor{blue}{1. q* should be related to the <Documents>, but the <Documents> can not provide any useful information for answering q*. \newline
2. a* should be able to answer q*, ensuring that the response a* is accurate, detailed, and comprehensive.} 
\newline

Additionally, to ensure diversity, richness, and high quality in the question q* you generate, we will randomly provide a question for you to emulate. In other words, while satisfying the requirements above, make q* similar in task requirement and expression to the \textcolor{darkred}{<Simulated Instruction>} below:  

\textcolor{darkred}{
<Simulated Instruction> \newline
\texttt{\{<Simulated Instruction>\}} \newline
</Simulated Instruction> \newline
}

Please directly generate the question-answer pair (q*, a*) following all the rules above in the format of \{"q*": ..., "a*": ...\}. Ensure the quality of the generated (q*, a*).
\end{prompt}
\caption{The prompt for synthesizing Useless Doc ($r_0$) data.}
\label{tab:r_0}
\end{figure*}

\begin{figure*}
\begin{prompt}[title={Single-Doc Support ($r_1$)}]\label{prompt_r3}
<Documents> \newline
[1] \texttt{\{<Document 1>\}}\newline
</Documents> \newline

Your task is to generate an English question q* and a corresponding response a* based on the provided <Documents>. Please note that the question q* can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats. You need to follow the requirements below to generate the q* and a* \textcolor{blue}{(RAG Paradigms)}:  

\textcolor{blue}{1. <Documents> can support q* by providing useful information or hints, but they do not contain explicit answers.\newline
2. a* should use useful information from <Documents> to aid in answering q*, ensuring that the response is accurate, detailed, and comprehensive.} 
\newline

Additionally, to ensure diversity, richness, and high quality in the question q* you generate, we will randomly provide a question for you to emulate. In other words, while satisfying the requirements above, make q* similar in task requirement and expression to the \textcolor{darkred}{<Simulated Instruction>} below:  

\textcolor{darkred}{
<Simulated Instruction> \newline
\texttt{\{<Simulated Instruction>\}} \newline
</Simulated Instruction> \newline
}

Please directly generate the question-answer pair (q*, a*) following all the rules above in the format of \{"q*": ..., "a*": ...\}. Ensure the quality of the generated (q*, a*).
\end{prompt}
    \caption{The prompt for synthesizing Single-Doc Support ($r_1$) data.}
\label{tab:r_1}
\end{figure*}

\begin{figure*}

\begin{prompt}[title={Multi-Doc Support ($r_2$)}] \label{prompt_r2}
<Documents> \newline
[1] \texttt{\{<Document 1>\}}\newline
[2] \texttt{\{<Document 2>\}} \newline
[3] ...\newline
</Documents> \newline

Your task is to generate an English question q* and a corresponding response a* based on the provided <Documents>. Please note that the question q* can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats. You need to follow the requirements below to generate the q* and a* \textcolor{blue}{(RAG Paradigms)}:  

\textcolor{blue}{1. Multiple documents within <Documents> can support q* by providing useful information or hints, but they do not contain explicit answers. \newline
2. a* should use useful information from <Documents> to aid in answering q*, ensuring that the response is accurate, detailed, and comprehensive.} 
\newline

Additionally, to ensure diversity, richness, and high quality in the question q* you generate, we will randomly provide a question for you to emulate. In other words, while satisfying the requirements above, make q* similar in task requirement and expression to the \textcolor{darkred}{<Simulated Instruction>} below:  

\textcolor{darkred}{
<Simulated Instruction> \newline
\texttt{\{<Simulated Instruction>\}} \newline
</Simulated Instruction> \newline
}

Please directly generate the question-answer pair (q*, a*) following all the rules above in the format of \{"q*": ..., "a*": ...\}. Ensure the quality of the generated (q*, a*).
\end{prompt}
     \caption{The prompt for synthesizing Multi-Doc Support ($r_2$) data.}
\label{tab:r_2}
\end{figure*}

\begin{figure*}
 
\begin{prompt}[title={Single-Doc Answer ($r_3$)}]\label{prompt_r3}
<Documents> \newline
[1] \texttt{\{<Document 1>\}}\newline
</Documents> \newline

Your task is to generate an English question q* and a corresponding response a* based on the provided <Documents>. Please note that the question q* can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats. You need to follow the requirements below to generate the q* and a* \textcolor{blue}{(RAG Paradigms)}:  

\textcolor{blue}{1. Ensure that q* can be answered directly using the content of <Documents>, meaning its answer can be fully derived from <Documents>. \newline
2. a* should use the information from <Documents> to answer q* accurately, ensuring that the response is accurate, detailed, and comprehensive.} 
\newline

Additionally, to ensure diversity, richness, and high quality in the question q* you generate, we will randomly provide a question for you to emulate. In other words, while satisfying the requirements above, make q* similar in task requirement and expression to the \textcolor{darkred}{<Simulated Instruction>} below:  

\textcolor{darkred}{
<Simulated Instruction> \newline
\texttt{\{<Simulated Instruction>\}} \newline
</Simulated Instruction> \newline
}

Please directly generate the question-answer pair (q*, a*) following all the rules above in the format of \{"q*": ..., "a*": ...\}. Ensure the quality of the generated (q*, a*).
\end{prompt}
    \caption{The prompt for synthesizing Single-Doc Answer ($r_3$) data.}
\label{tab:r_3}
\end{figure*}

\begin{figure*}
 
\begin{prompt}[title={Multi-Doc Answer ($r_4$)}]
\label{prompt_r4}
<Documents> \newline
[1] \texttt{\{<Document 1>\}}\newline
[2] \texttt{\{<Document 2>\}} \newline
[3] ...\newline
</Documents> \newline

Your task is to generate an English question q* and a corresponding response a* based on the provided <Documents>. Please note that the question q* can take various forms, not limited to questions with a question mark, but also including statements, instructions, and other formats. You need to follow the requirements below to generate the q* and a* \textcolor{blue}{(RAG Paradigms)}:  

\textcolor{blue}{1. The answer to q* can be derived from multiple documents within <Documents>, involving multi-hop reasoning or the integration of information from several documents. \newline
2. a* should leverage the information in <Documents> to provide an accurate answer to q*, ensuring that the response is accurate, detailed, and comprehensive.} 
\newline

Additionally, to ensure diversity, richness, and high quality in the question q* you generate, we will randomly provide a question for you to emulate. In other words, while satisfying the requirements above, make q* similar in task requirement and expression to the \textcolor{darkred}{<Simulated Instruction>} below:  

\textcolor{darkred}{
<Simulated Instruction> \newline
\texttt{\{<Simulated Instruction>\}} \newline
</Simulated Instruction> \newline
}

Please directly generate the question-answer pair (q*, a*) following all the rules above in the format of \{"q*": ..., "a*": ...\}. Ensure the quality of the generated (q*, a*).
\end{prompt}
      \caption{The prompt for synthesizing Multi-Doc Answer ($r_4$) data.}
\label{tab:r_4}
\end{figure*}
